Improved sampling algorithms and functional inequalities for non-log-concave distributions

We study the problem of sampling from a distribution $\mu$ with density $\propto e^{-V}$ for some potential function $V:\mathbb R^d\to \mathbb R$ with query access to $V$ and $\nabla V$. We start with the following standard assumptions: (1) $V$ is $L$-smooth. (2) The second moment $\mathbf{E}_{X\sim \mu}[\|X\|^2]\leq M$. Recently, He and Zhang (COLT'25) showed that the query complexity of this problem is at least $\left(\frac{LM}{d\epsilon}\right)^{\Omega(d)}$ where $\epsilon$ is the desired accuracy in total variation distance, and the Poincar\'e constant can be unbounded. Meanwhile, another common assumption in the study of diffusion based samplers (see e.g., the work of Chen, Chewi, Li, Li, Salim and Zhang (ICLR'23)) strengthens (1) to the following: (1*) The potential function of *every* distribution along the Ornstein-Uhlenbeck process starting from $\mu$ is $L$-smooth. We show that under the assumptions (1*) and (2), the query complexity of sampling from $\mu$ can be $\mathrm{poly}(L,d)\cdot \left(\frac{Ld+M}{\epsilon^2}\right)^{\mathcal{O}(L+1)}$, which is polynomial in $d$ and $\frac{1}{\epsilon}$ when $L=\mathcal{O}(1)$ and $M=\mathrm{poly}(d)$. This improves the algorithm with quasi-polynomial query complexity developed by Huang et al. (COLT'24). Our results imply that the seemingly moderate strengthening from (1) to (1*) yields an exponential gap in the query complexity. Furthermore, we show that together with the assumption (1*) and the stronger moment assumption that $\|X\|$ is $\lambda$-sub-Gaussian for $X\sim\mu$, the Poincar\'e constant of $\mu$ is at most $\mathcal{O}(\lambda)^{2(L+1)}$. We also establish a modified log-Sobolev inequality for $\mu$ under these conditions. As an application of our technique, we obtain a new estimate of the modified log-Sobolev constant for a specific class of mixtures of strongly log-concave distributions.

==> figure.tex <==

%<*SLfigure>
% Gradient Info
  
\tikzset {_btr2zfapx/.code = {\pgfsetadditionalshadetransform{ \pgftransformshift{\pgfpoint{0 bp } { 0 bp }  }  \pgftransformrotate{0 }  \pgftransformscale{2 }  }}}
\pgfdeclarehorizontalshading{_ahsjayvuf}{150bp}{rgb(0bp)=(1,1,1);
rgb(40.17857142857143bp)=(1,1,1);
rgb(52.767857142857146bp)=(0.5,0.5,0.5);
rgb(54.375bp)=(0.5,0.5,0.5);
rgb(60.535714285714285bp)=(0,0,0);
rgb(100bp)=(0,0,0)}
\tikzset{_jnp66vckz/.code = {\pgfsetadditionalshadetransform{\pgftransformshift{\pgfpoint{0 bp } { 0 bp }  }  \pgftransformrotate{0 }  \pgftransformscale{2 } }}}
\pgfdeclarehorizontalshading{_cq9p49t32} {150bp} {color(0bp)=(transparent!0);
color(40.17857142857143bp)=(transparent!0);
color(52.767857142857146bp)=(transparent!0);
color(54.375bp)=(transparent!0);
color(60.535714285714285bp)=(transparent!10);
color(100bp)=(transparent!10) } 
\pgfdeclarefading{_g6tclfbm0}{\tikz \fill[shading=_cq9p49t32,_jnp66vckz] (0,0) rectangle (50bp,50bp); } 

% Gradient Info
  
\tikzset {_1k7orc7e5/.code = {\pgfsetadditionalshadetransform{ \pgftransformshift{\pgfpoint{0 bp } { 0 bp }  }  \pgftransformrotate{0 }  \pgftransformscale{2 }  }}}
\pgfdeclarehorizontalshading{_qqwtkblrs}{150bp}{rgb(0bp)=(0.6,0.85,1);
rgb(37.5bp)=(0.6,0.85,1);
rgb(62.5bp)=(0,0.5,0.5);
rgb(100bp)=(0,0.5,0.5)}
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Rectangle [id:dp292785154219796] 
\draw  [draw opacity=0][shading=_ahsjayvuf,_btr2zfapx,path fading= _g6tclfbm0 ,fading transform={xshift=2}] (73,143.33) -- (601.67,143.33) -- (601.67,146.13) -- (73,146.13) -- cycle ;
%Straight Lines [id:da8359363412861076] 
\draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][shading=_qqwtkblrs,_1k7orc7e5][line width=0.75]    (73,143.5) -- (189.67,143.5) -- (601,143.5)(73,146.5) -- (189.67,146.5) -- (601,146.5) ;
\draw [shift={(610,145)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Shape: Circle [id:dp36390254001323885] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (70.13,145) .. controls (70.13,143.41) and (71.41,142.13) .. (73,142.13) .. controls (74.59,142.13) and (75.88,143.41) .. (75.88,145) .. controls (75.88,146.59) and (74.59,147.88) .. (73,147.88) .. controls (71.41,147.88) and (70.13,146.59) .. (70.13,145) -- cycle ;
%Shape: Circle [id:dp5267559355386695] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (116.13,144.88) .. controls (116.13,143.29) and (117.41,142) .. (119,142) .. controls (120.59,142) and (121.88,143.29) .. (121.88,144.88) .. controls (121.88,146.46) and (120.59,147.75) .. (119,147.75) .. controls (117.41,147.75) and (116.13,146.46) .. (116.13,144.88) -- cycle ;
%Shape: Circle [id:dp46120604028733037] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (461.73,144.6) .. controls (461.73,143.01) and (463.01,141.73) .. (464.6,141.73) .. controls (466.19,141.73) and (467.48,143.01) .. (467.48,144.6) .. controls (467.48,146.19) and (466.19,147.48) .. (464.6,147.48) .. controls (463.01,147.48) and (461.73,146.19) .. (461.73,144.6) -- cycle ;
%Straight Lines [id:da0011250900590827895] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (73,147.88) -- (73,169.38) ;
%Straight Lines [id:da2276393529583277] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (119,147.75) -- (119,169.25) ;
%Straight Lines [id:da7732630968014685] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (464.6,147.48) -- (464.6,168.98) ;
%Shape: Brace [id:dp08690475372190576] 
\draw   (455.5,119) .. controls (455.5,114.33) and (453.17,112) .. (448.5,112) -- (301.5,112) .. controls (294.83,112) and (291.5,109.67) .. (291.5,105) .. controls (291.5,109.67) and (288.17,112) .. (281.5,112)(284.5,112) -- (129.5,112) .. controls (124.83,112) and (122.5,114.33) .. (122.5,119) ;
%Rounded Rect [id:dp9567374173332546] 
\draw  [dash pattern={on 0.84pt off 2.51pt}] (24,97.6) .. controls (24,84.01) and (35.01,73) .. (48.6,73) -- (612.4,73) .. controls (625.99,73) and (637,84.01) .. (637,97.6) -- (637,171.4) .. controls (637,184.99) and (625.99,196) .. (612.4,196) -- (48.6,196) .. controls (35.01,196) and (24,184.99) .. (24,171.4) -- cycle ;


% Text Node
\draw (40,169) node [anchor=north west][inner sep=0.75pt]    {$\mu =\nu _{0}$};
% Text Node
\draw (112,169) node [anchor=north west][inner sep=0.75pt]    {$\nu _{s_{0}}$};
% Text Node
\draw (458,169) node [anchor=north west][inner sep=0.75pt]    {$\nu _{T}$};
% Text Node
\draw (67,122.4) node [anchor=north west][inner sep=0.75pt]    {$0$};
% Text Node
\draw (114,123.5) node [anchor=north west][inner sep=0.75pt]    {$s_{0}$};
% Text Node
\draw (459,122.4) node [anchor=north west][inner sep=0.75pt]    {$T$};
% Text Node
\draw (89.5,169) node [anchor=north west][inner sep=0.75pt]    {$\approx $};
% Text Node
\draw (557,174.4) node  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ] [align=left] {\begin{minipage}[lt]{115.94pt}\setlength\topsep{0pt}
: strongly log-concave
\end{minipage}};
% Text Node
\draw (175,82.4) node [anchor=north west][inner sep=0.75pt]    {$\forall \ s\in [ s_{0} ,T] ,\ \mathrm{cov}( \nu _{s})$};
% Text Node
\draw (393,90.4) node   [align=left] {\begin{minipage}[lt]{115.94pt}\setlength\topsep{0pt}
is bounded
\end{minipage}};


\end{tikzpicture}
%</SLfigure>
